Ranking with Slot Constraints

We introduce the problem of ranking with slot constraints, which can be used to model a wide range of application problems -- from college admission with limited slots for different majors, to composing a stratified cohort of eligible participants in a medical trial. We show that the conventional Probability Ranking Principle (PRP) can be highly sub-optimal for slot-constrained ranking problems, and we devise a new ranking algorithm, called MatchRank. The goal of MatchRank is to produce rankings that maximize the number of filled slots if candidates are evaluated by a human decision maker in the order of the ranking. In this way, MatchRank generalizes the PRP, and it subsumes the PRP as a special case when there are no slot constraints. Our theoretical analysis shows that MatchRank has a strong approximation guarantee without any independence assumptions between slots or candidates. Furthermore, we show how MatchRank can be implemented efficiently. Beyond the theoretical guarantees, empirical evaluations show that MatchRank can provide substantial improvements over a range of synthetic and real-world tasks.

==> computational_efficiency.tex <==
\subsection{Computational Efficiency of \algname and Improvements} \label{sec:efficiency}

The \algname algorithm as written in \alg{alg:greedy} is optimized for clarity, but there are a number of improvements that can substantially speed up computation. To motivate these improvements, we first analyze the runtime complexity of \alg{alg:greedy}.

For computing the top $k$ positions of the ranking when there are $\CandidatesNum$ candidates, $\SlotsNum$ slots, and $\n$ Monte-Carlo samples, the greedy maximizer inside \alg{alg:greedy} will evaluate $O(k \, \CandidatesNum)$ sets. For each such set, it will find the MBM solutions of all bipartite graphs from $\RelSamples$, which takes $\n \, O(\CandidatesNum \, \SlotsNum \, \sqrt{\CandidatesNum + \SlotsNum})$ time per set when using the classic Hopcroft-Karp MBM algorithm \cite{hopcroft1973n}. So, a naive implementation will take $O(k \, \n \, \CandidatesNum^2 \, \SlotsNum \, \sqrt{\CandidatesNum + \SlotsNum})$ time. However, this implementation is unnecessarily slow.



We can improve the time efficiency of \textit{MatchRank} by following the principle that any unmatched candidate can increase the matching size by at most 1. So, if we are given a candidate set $\candset \subseteq \Candidates$ and an unmatched candidate $\cand$, finding the $\mbm{\candset \cup \{\cand \}}{\Slots}{\Rel}$ can be reduced to determining if there is an augmenting path to the matching of $\mbm{\candset}{\Slots}{\Rel}$ starting from $\cand$. If such an augmenting path exists, then we can extend the matching and $\mbm{\candset \cup \{\cand \}}{\Slots}{\Rel} = \mbm{\candset}{\Slots}{\Rel} + 1$. It no augmenting path exists, then we will know that $\mbm{\candset \cup \{\cand \}}{\Slots}{\Rel}=\mbm{\candset}{\Slots}{\Rel}$ and the matching remains unchanged. Therefore, it will take $O(\CandidatesNum \, \SlotsNum)$ time (a BFS) per each unmatched candidate per ranking step, and we obtain an $O(k \, \n \, \CandidatesNum \, (\CandidatesNum \, \SlotsNum)) = O(k \, \n \, \CandidatesNum^2 \, \SlotsNum)$ algorithm.  

If we consider the typical scenario where $\CandidatesNum > \SlotsNum$, we can improve the time complexity by keeping a list of unmatched slots instead of candidates for each bipartite graph, and on each ranking step we start from each unmatched slot and follow the BFS to find all augmenting paths that end on unmatched candidates. We require $O(\CandidatesNum \, \SlotsNum^2)$ time per ranking step, and in total only $O(k \, \n \, \CandidatesNum \, \SlotsNum^2)$ time.  

%  \begin{theorem}
%     \textit{MatchRank} can be implemented to run with worst-case time complexity of $O(k \, \n \, \CandidatesNum \, \SlotsNum^2)$ for rankings of length $k$ with $\CandidatesNum$ candidates, $\SlotsNum \le \CandidatesNum$ slots, and $\n$ Monte-Carlo samples.
%     \label{lem:time}
% \end{theorem}

% \begin{proof}
%     Given a ranking shortlist $\candset \subseteq \Candidates$ and slots $\Slots$, an unmatched candidate (free vertex) $\cand \in \Candidates - \candset$, $\cand$ can at most increase the matching size by 1 after adding to $\candset$. So, we only have to determine if there is an augmenting path starting from $\cand$ to  $\mbm{\candset}{\Slots}{\Rel}$. 

% \end{proof}


A further improvement in runtime can be achieved by exploiting that \algname is a greedy algorithm for maximizing a submodular objective. For any such algorithm, we can use lazy evaluation \cite{minoux1978accelerated} to accelerate the ranking process in practice\footnote{We run all of our experiments with lazy greedy.}. Lazy greedy maintains a priority queue of stale marginal gains to reduce unnecessary computation of marginal gains for many examples per step. Since marginal gains can never increase due to the submodularity of the objective, the stale marginal gains provide an upper bound on the improvement. Thus, if a stale marginal gain is not large enough to propose a candidate as a greedy maximizer, then recomputing its marginal gain is not necessary. This is particularly effective in our matching scenarios, since many candidates are not relevant for some slots. This means they will have small marginal gains even in the first step of ranking, and we can significantly reduce computation of their marginal gains during subsequent iterations when using lazy greedy.

Finally, we could replace the greedy algorithm with some approximate version of greedy that is substantially faster, such as stochastic greedy \cite{mirzasoleiman2015lazier} and threshold greedy \cite{badanidiyuru2014fast} for monotone submodular maximization problem. We have performed initial evaluations of these methods with promising results, but did not find a need for them for our experiments. Generally, we found the exact greedy algorithm to be tractable for datasets with up to 50,000 candidates. 


==> sections/problem-settings/problem-settings.tex <==

Much work on ranking focuses on finding results that are relevant to a single query. However, often a user has multiple interrelated information needs, or seeks a set of results that contain complementary content. For example, in hiring and admissions, one seeks an assignment from applicants to roles, where items may be qualified for multiple roles. In recommendations, one may want to show a selection of items that cover a range of categories (movie genres, individual articles of clothing that would work together in an outfit). In these cases, it may not suffice to show separate rankings for different queries due to the dependencies between results -- choosing a particular item from one category may affect the best item of another, because items could belong to multiple categories.

A specific use of this algorithm could be in college admissions or hiring. This is inspired by the Rooney Rule, but our algorithm will allows far greater complexity in the evaluation process. To use admissions as an example, as the very first stage in the admission process, the admissions officer may decide that they want to interview $n_1$ applicants for the CS major, $n_2$ students for ECE, $n_3$ students for the hockey team, etc. This means there would be $m_1$ CS slots, $m_2$ ECE slots, $m_3$ hockey slots, etc. The goal is to fill these slots with interview candidates so that we maximize the expected number of "successful" interviews (i.e. interviews that surface a candidate that is qualified for admission). At a high level, this goal is consistent with using the available reviewing resources (e.g. number of interviews that can be conducted) in the most effective way subject to the slot constraints.

\input{diagram/dataflow.tex}

We define the setting as follows. A set of $n$ items $A$ is to be assigned to a set of $m$ slots $S$. There's a qualification matrix $\Q \in \mathbb{R}^{n \times m}$ that gives the affinity of an item to a particular slot. For now, assume the entries of $\Q$ are binary, in which $\Q[a, s] = 1$ means item $a$ is qualified for slot $s$ and $0$ otherwise. $\Q$ is unknown apriori, but the distribution $\PQ$ is known, or can be approximated by $\hat{P}(Q)$ from some regression models. We wish to output a ranking $C \subseteq A$ of the items so that given a prefix of $k$ items from the ranking, the excepted value (w.r.t. $\PQ$) of the matched slots from qualified items in the prefix to slots is maximized, i.e. we want to maximize $\mathbb{E}_{\Q \sim \PQ}[\sum_{a, s \in Q(C_k, S)} Q_{a,s}]$ for a ranking $C$ and all prefix $k$.


